Predictive Coding-based Deep Neural Network Fine-tuning for Computationally Efficient Domain Adaptation

As deep neural networks are increasingly deployed in dynamic, real-world environments, relying on a single static model is often insufficient. Changes in input data distributions caused by sensor drift or lighting variations necessitate continual model adaptation. In this paper, we propose a hybrid training methodology that enables efficient on-device domain adaptation by combining the strengths of Backpropagation and Predictive Coding. The method begins with a deep neural network trained offline using Backpropagation to achieve high initial performance. Subsequently, Predictive Coding is employed for online adaptation, allowing the model to recover accuracy lost due to shifts in the input data distribution. This approach leverages the robustness of Backpropagation for initial representation learning and the computational efficiency of Predictive Coding for continual learning, making it particularly well-suited for resource-constrained edge devices or future neuromorphic accelerators. Experimental results on the MNIST and CIFAR-10 datasets demonstrate that this hybrid strategy enables effective adaptation with a reduced computational overhead, offering a promising solution for maintaining model performance in dynamic environments.

==> images_layers_init.tex <==
% ------------------------------------------------------------------------------
% This file is a modified version of layers/init.tex from PlotNeuralNet
%   Original repository: https://github.com/HarisIqbal88/PlotNeuralNet
% ------------------------------------------------------------------------------
%
% MIT License
%
% Copyright (c) 2018 HarisIqbal88
%
% Permission is hereby granted, free of charge, to any person obtaining a copy
% of this software and associated documentation files (the "Software"), to deal
% in the Software without restriction, including without limitation the rights
% to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
% copies of the Software, and to permit persons to whom the Software is
% furnished to do so, subject to the following conditions:
%
% The above copyright notice and this permission notice shall be included in all
% copies or substantial portions of the Software.
%
% THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
% IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
% FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
% AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
% LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
% OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN THE
% SOFTWARE.
%
% ------------------------------------------------------------------------------
%
% Modified by: Matteo Cardoni, 2025
% ------------------------------------------------------------------------------

\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\providecommand{\midarrow}{\tikz \draw[-Stealth,line width =1.5mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{images_layers_box}


==> plots_lib_accuracy_plot.tex <==
\providecommand{\plotAcc}[7]{%
  \pgfplotstableread[col sep=comma]{#1}\datatable

  \addplot[
    color=#4,
    draw,
    legend image post style={line width=1.5pt},
    #7
  ] table[x expr=(\thisrow{epoch}+1)*#2, y expr=(\thisrowno{1})*#3]{\datatable};

  \ifthenelse{\equal{#5}{true}}{
    \addlegendentry{#6}
  }{
  }%
}


==> plots_lib_init.tex <==
\usepackage{ifthen}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usetikzlibrary{intersections}
\usepgfplotslibrary{fillbetween}
\pgfplotsset{compat=1.18}
\usepackage{subcaption}
\usepackage{mwe}
\usepackage{import}
\usepackage[dvipsnames]{xcolor}

\import{}{plots_lib_mean_stddev_plot}
\import{}{plots_lib_accuracy_plot}

